Placing the spotted T Tauri star LkCa 4 on an HR diagram

Ages and masses of young stars are often estimated by comparing their luminosities and effective temperatures to pre-main sequence stellar evolution tracks, but magnetic fields and starspots complicate both the observations and evolution. To understand their influence, we study the heavily-spotted weak-lined T-Tauri star LkCa 4 by searching for spectral signatures of radiation originating from the starspot or starspot groups. We introduce a new methodology for constraining both the starspot filling factor and the spot temperature by fitting two-temperature stellar atmosphere models constructed from Phoenix synthetic spectra to a high-resolution near-IR IGRINS spectrum. Clearly discernable spectral features arise from both a hot photospheric component $T_{\mathrm{hot}} \sim4100$ K and to a cool component $T_{\mathrm{cool}} \sim2700-3000$ K, which covers $\sim80\%$ of the visible surface. This mix of hot and cool emission is supported by analyses of the spectral energy distribution, rotational modulation of colors and of TiO band strengths, and features in low-resolution optical/near-IR spectroscopy. Although the revised effective temperature and luminosity make LkCa 4 appear much younger and lower mass than previous estimates from unspotted stellar evolution models, appropriate estimates will require the production and adoption of spotted evolutionary models. Biases from starspots likely afflict most fully convective young stars and contribute to uncertainties in ages and age spreads of open clusters. In some spectral regions starspots act as a featureless veiling continuum owing to high rotational broadening and heavy line-blanketing in cool star spectra. Some evidence is also found for an anti-correlation between the velocities of the warm and cool components.

==> setup.tex <==
%% For anyone who downloaded my source file from arxiv:
%% I stole most of this setup.tex from a paper by Peter .K.G. Williams, but I made a bunch of edits to satisfy my own needs. You might check his paper out (http://arxiv.org/abs/1409.4411) for the original source file or contact him if you have any questions, since I don't really understand how some of these things work. 
%One cool thing it does is you can define an object, just that when someone clicks on the pdf it will link to simbad. I could never quite get this to work, probably because you have to get the text exactly right and my motivation for getting it to work was not super high. 


% basic packages
\usepackage{amsmath,amssymb}
\usepackage[breaklinks,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
\usepackage{epsfig}    
\usepackage{graphicx}    
\usepackage{lineno}
\usepackage{natbib}
\usepackage{bigints}
\usepackage[outdir=./]{epstopdf}



% font stuff
\usepackage[T1]{fontenc}
\pwifjournal\else
  \usepackage{microtype}
\fi


% emulateapj has overly conservative figure widths, I think because some
% people's figures don't have good margins. Override.
\pwifjournal\else
  \makeatletter
  \renewcommand\plotone[1]{%
    \centering \leavevmode \setlength{\plot@width}{0.95\linewidth}
    \includegraphics[width={\eps@scaling\plot@width}]{#1}%
  }%
  \makeatother
\fi


\makeatletter

\newcommand\@simpfx{http://simbad.u-strasbg.fr/simbad/sim-id?Ident=}

\newcommand\MakeObj[4][\@empty]{% [shortname]{ident}{url-escaped}{formalname}
  \pwifjournal%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\protect\object[#4]{##1}}%
  \else%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\href{\@simpfx #3}{##1}}%
  \fi%
  \expandafter\newcommand\csname pkgwobj@f#2\endcsname{#4}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#4}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%

\newcommand\MakeTrunc[2]{% {ident}{truncname}
  \expandafter\newcommand\csname pkgwobj@t#1\endcsname{#2}}%

\newcommand{\obj}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@s#1\endcsname}%
  \fi}
\newcommand{\objf}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@f#1\endcsname}%
  \fi}
\newcommand{\objt}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@t#1\endcsname}%
  \fi}

\makeatother


% Evil magic to patch natbib to only highlight the year paper refs, not the
% authors too; as seen in ApJ. From
% http://tex.stackexchange.com/questions/23227/.

\pwifjournal\else
  \usepackage{etoolbox}
  \makeatletter
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
         {\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
    {}{}
  \makeatother
\fi


% Object data
\MakeObj{n33370}{NLTT\%2033370}{NLTT~33370\,AB}
\MakeTrunc{n33370}{NLTT~33370}
\MakeObj{tvlm}{TVLM\%20513-46546}{TVLM~513--46546}

% utility

\newcommand{\vdag}{(v)^\dagger}
\newcommand{\oxygen}{O$_2$}
\newcommand{\water}{H$_2$O}
\newcommand{\kepler}{{\it Kepler}}
\newcommand{\logg}{$log~g$ }
\newcommand{\metal}{[M/H]}
\newcommand{\um}{$\mu$m}
\newcommand{\fbol}{$F_{\mathrm{bol}}$}
\newcommand{\mbol}{$m_{\mathrm{bol}}$}
\newcommand{\Mbol}{$M_{\mathrm{bol}}$}
\newcommand{\rapsq}{$R_{ap}^2$}
\newcommand{\rchisq}{$\chi^2_{\nu}$}
\newcommand{\hipp}{{\it Hipparcos}}


\newcommand\aafd{erg~s$^{-1}$~cm$^{-2}$~\AA$^{-1}$} % "AAngstrom flux density"
\newcommand\amlt{$\alpha_{\rm MLT}$} % convective mixing length parameter
\newcommand\apx{\ensuremath{\sim}}
\newcommand\cgsflux{erg~s$^{-1}$~cm$^{-2}$}
\newcommand\cgslum{erg~s$^{-1}$}
\newcommand\chandra{\textit{Chandra}}
\newcommand\citeeg[1]{\citep[\eg,][]{#1}}
\newcommand\cps{ct~s$^{-1}$}
\newcommand\dd{\ensuremath{\text{d}}}
\newcommand\eg{\textit{e.g.}}
\newcommand\etal{\textit{et~al.}}
\newcommand\ewha{\ensuremath{\text{EW}(\ha)}}
\newcommand\fig[1]{Figure~\ref{f.#1}}
\newcommand\ha{{\ensuremath{\text{H}\alpha}}}
\newcommand\I{\mathcal{I}}
\newcommand\ie{\textit{i.e.}}
\newcommand\kms{km~s$^{-1}$}
\newcommand\ls{L$_\odot$}
\newcommand\mj{M$_\text{J}$}
\newcommand\ms{M$_\odot$}
\newcommand\nupk{\ensuremath{\nu_\text{pk}}}
\newcommand\percc{cm$^{-3}$}
\newcommand\rcs{\ensuremath{\chi_r^2}}
\newcommand\rj{R$_\text{J}$}
\newcommand\sect[1]{Section~\ref{s.#1}}
\newcommand\sherpa{\textsf{Sherpa}}
\newcommand\sti{Stokes~$I$}
\newcommand\stiv{Stokes~$I$ and~$V$}
\newcommand\stv{Stokes~$V$}
\newcommand\swift{\textit{Swift}}
\newcommand\tb{\ensuremath{T_\text{b}}}
\newcommand\tbl[1]{Table~\ref{t.#1}}
\newcommand\teff{\ensuremath{T_\text{eff}}}
\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand\ujy{$\mu$Jy}
\newcommand\ujybm{$\mu$Jy~bm$^{-1}$}
\newcommand\uv{$u$\mbox{-}$v$}
\newcommand\vsi{\ensuremath{v \sin i}}

\newcommand\Lb{\ensuremath{L_\text{bol}}}
\newcommand\Lh{\ensuremath{L_\ha}}
\newcommand\Lr{\ensuremath{L_\text{R}}}
\newcommand\sLr{\ensuremath{L_{\nu,\text{R}}}}
\newcommand\Lu{\ensuremath{L_\text{UVW1}}}
\newcommand\Lx{\ensuremath{L_\text{X}}}
\newcommand\Lxf{\ensuremath{L_{\text{X},f}}}
\newcommand\Lxq{\ensuremath{L_{\text{X},q}}}
\newcommand\lb{\ensuremath{[\Lb]}}
\newcommand\lh{\ensuremath{[\Lh]}}
\newcommand\lr{\ensuremath{[\Lr]}}
\newcommand\slr{\ensuremath{[\sLr]}}
\newcommand\lu{\ensuremath{[\Lu]}}
\newcommand\lx{\ensuremath{[\Lx]}}
\newcommand\lxf{\ensuremath{[\Lxf]}}
\newcommand\lxq{\ensuremath{[\Lxq]}}
\newcommand\lhlb{\ensuremath{[\Lh/\Lb]}}
\newcommand\lrlb{\ensuremath{[\Lr/\Lb]}}
\newcommand\lulb{\ensuremath{[\Lu/\Lb]}}
\newcommand\lxlb{\ensuremath{[\Lx/\Lb]}}
\newcommand\lxflb{\ensuremath{[\Lxf/\Lb]}}
\newcommand\lxqlb{\ensuremath{[\Lxq/\Lb]}}
\newcommand\slrlb{\ensuremath{[\sLr/\Lb]}}
\newcommand\slrlx{\ensuremath{[\sLr/\Lx]}}
\newcommand\slrlxf{\ensuremath{[\sLr/\Lxf]}}
\newcommand\slrlxq{\ensuremath{[\sLr/\Lxq]}}

